Fano varieties in Mori fibre spaces

We show that being a general fibre of a Mori fibre space is a rather restrictive condition for a Fano variety. More specifically, we obtain two criteria (one sufficient and one necessary) for a Q-factorial Fano variety with terminal singularities to be realised as a fibre of a Mori fibre space, which turn into a characterisation in the rigid case. We apply our criteria to figure out this property up to dimension three and on rational homogeneous spaces. The smooth toric case is studied and an interesting connection with K-semistability is also investigated.

==> sec_toric.tex <==
\section{$K$-stability in the smooth toric case}
\label{sec_toric}


%In this section we will deal with smooth toric Fano varieties. We will give evidence of what we expect to be a general picture for smooth Fano varieties: fibre-likeness should imply $K$-semistability. 

%INVECE DI QUESTA COSA VAGA SCRIVEREI 

In this section we prove that any smooth fibre-like toric Fano variety has barycentre in the origin (i.e. it is $K$-stable). Let us point out that there are smooth toric varieties that are $K$-stable but not fibre-like, such as $\pp^1\times \pp^2$. 


%The toric hypothesis allows us to translate many deep geometric properties into pure combinatorial data on the polytope. For instance, 












%MI PARE CI FOSSE L'ESEMPIO DI UN SPAZIO PROIETTIVO PESATO FIBRE-LIKE CHE NON ERA K STABILE E NON AVEVA IL BARICENTRO NELL'ORIGINE. FORSE VALE LA PENA DIRLO.

\subsection{Preliminaries on toric geometry: primitive collections}

We start recalling some notation and basic facts. For more details, see \cite{CLS11}, \cite{Bat91} and \cite{Cas03a}.

Let $N$ be a free abelian group of rank $n$ and set $N_\qq:=N\otimes_\zz \qq$. Denote by $M$ the dual of $N$.  Let $\Sigma \subset N_\qq$ be a fan of an $n$-dimensional smooth toric Fano variety $F$ and let $\De \subset N_\qq$ be the dual polytope associated to the anti-canonical polarisation. 

The vertices of $\De$, denoted by $V(\De)$, are the generators of $\Sigma$. %We denote by $Z(\sigma)$ the closure of the orbit corresponding to $\sigma\in \Sigma$, which is an irreducible invariant subvariety.

Let $N_1$ be the group of 1-cycles on $F$ modulo numerical equivalence and set $(N_1)_\qq=N_1 \otimes \qq$. In $N_1(F)_\qq$ we consider the Kleiman-Mori cone $\NE(F)$ generated  by the effective 1-cycles. There is the following basic exact sequence:
\begin{equation}\label{toricses1}
0 \rightarrow N_1(F) \rightarrow \zz^{V(\De)}\rightarrow N \rightarrow 0
\end{equation}
and dually
\begin{equation}\label{toricses2}
0 \rightarrow M \rightarrow \zz^{V(\De)}\rightarrow N^1(F) \rightarrow 0.
\end{equation}

In this subsection, we also need some notation and results about primitive collections.

\begin{definition}
A subset $\mathcal P \subset V(\Delta)$ is called a \emph{primitive collection} if the cone generated by $\mathcal  P$ is not in $\Sigma$, while for each $x \in \mathcal  P$ the elements of $\mathcal  P \setminus \{x\}$ generate a cone in $\Sigma$. 
\end{definition}
For a primitive collection $\mathcal  P=\{x_1, \ldots,x_k\}$ denote by $\sigma(\mathcal  P)$ the (unique) minimal cone in $\Sigma$ such that $(x_1+\ldots +x_k) \in \sigma(\mathcal  P)$ . Let $y_1,\ldots,y_h$ be generators of $\sigma(\mathcal  P)$. Then we have
$$
r(P)\colon x_1+\ldots +x_k=b_1y_1+\ldots +b_hy_h
$$
where $b_i$ are  positive integers.   
\begin{definition}
The linear relation $r(\mathcal  P)$ is called \emph{the primitive relation of $\mathcal  P$} and the cone $\sigma(\mathcal  P)$ is called the focus of $\mathcal  P$. 
The integer $k$ is called the {\it length of $r\mathcal  (P)$} and the {\it degree of $\mathcal  P$} is defined as $\deg \mathcal  P= k - \sum b_i$.
\end{definition}

%Note that for any subset $P \subset V(\De)$  we can define in the same way its focus $\sigma(P)$, its relation $r(P)$, its order and its degree (non capisco perche' non venga fatto in letteratura). 

Using the exact sequence (\ref{toricses1}) we have the following identification between $N_1$ and the group generated by relations among the vertexes of $\De$:
$$
N_1(F) \cong \left\lbrace (b_x)_{x \in V(\De)} \in \Hom(\zz^{m}, \zz)\   \Bigg| \ \sum_{x \in V(\De)} b_x x=0\right\rbrace .
$$

\begin{rem}
By abuse of notation we denote by $r(\mathcal  P)$ also the cycle associated, via the previous isomorphism, to the relation
$$
x_1+\ldots +x_k = (b_1y_1 + \ldots + b_hy_h).
$$ 
 Note that $\deg \mathcal  P = -(K_F \cdot r(\mathcal  P))$ and so, since we are considering Fano varieties, any primitive relation has strictly positive degree.
\end{rem}

%Let $P$ be a primitive collection such that $r(P)$ is {\it extremal} (i.e. it generates an extremal ray in $\NE(F)$). The exceptional locus of the associated contraction 
%$$\phi_P: F \to F_P$$
%is $Z(\sigma(P))$. 
%According to $\sigma(P)$, we obtain the different steps of the MMP.
%\begin{description}
%\item[Divisorial contraction] It appears when $\sigma(P)$ is a one-dimensional cone and the contracted divisor is precisely the one associated to the ray.
%\item[Mori fibre space] In this case $\sigma(P)$ is the origin.
%\item[Flipping contraction] This appears in all the other cases.
%\end{description} 

%If $\sigma(P)=0$, then $\phi_P$ is of fibre type and if $\sigma(P)=\langle y\rangle$, then $\phi_P$ is a divisorial contraction.

%NOTA: The cone $NE(\De)$ is generated by the primitive relations and the primitive relations completely determine the variety. 

We will need the following result (cf. \cite[Proposition 3.2]{Bat91}).

\begin{proposition}[Batyrev]\label{batyrev}
Let $F$ be a smooth toric Fano variety. Then there exists a primitive collection $\mathcal  P$ such that $\sigma(\mathcal  P)=0$.
\end{proposition}

\begin{rem}\label{rmk}
Let 
$$a_1x_1+\cdots+a_kx_k=b_1y_1+\cdots+b_hy_h$$
be a relation among vertices of $\De$ with all $\{a_i\}$ and $\{b_j\}$ positive integers. Assume that $\sum a_i \ge \sum b_j.$
Then, by Lemma 1.4 in \cite{Cas03a}, $\langle x_1\cdots, x_k\rangle \not\in \Sigma$.
\end{rem}


\subsection{Fibre-likeness implies $K$-stability}
It is known that the symmetry of the polytope $\Delta$ is strictly related to the $K$-stability, which is known to be equivalent to the existence of K\"ahler-Einstein metric (cf. \cite{WZ} and \cite{BB}) of the associated Fano variety. Mabuchi proved in \cite{mabuchi} the first result relating the $K$-stability with the triviality of the barycentre of $\Delta$. This result was generalised in the singular setting in \cite{Ber12}. 


\begin{theorem}[{\cite[Cor. 1.2]{Ber12}}]\label{berg}
Let $F(\Delta)$ be a Gorenstein toric Fano variety. Then $F$ is $K$-stable if and only if the barycentre of $\Delta$ is the origin.
\end{theorem}

The proof of the previous result is analytic and passes through the existence of K\"ahler-Einstein metrics. Applying the theorem above, we can see that there are Gorenstein terminal $\Q$-factorial  toric varieties which are fibre-like, but not $K$-stable, e.g. the weighted projective space $\mathbb P(1,1,1,1,2)$.


In this context our main result is the following.

\begin{theorem}\label{cor_kstability}
Every smooth toric fibre-like Fano variety $F(\Delta)$ has barycentre in the origin and, as a consequence, is $K$-stable.
\end{theorem}

Before proving the theorem, we need to recall some convex geometry.

\begin{remark}
A basic fact is the following: the intersection of a convex polytope with an affine space is again a convex polytope.
\end{remark}

\begin{lemma}\label{lemma_convex_1}
Let $P$ be an $n$-dimensional convex polytope in an affine space $W\simeq\qq^n$ and let $H$ be a $k$-dimensional affine subspace intersecting $P$ in its interior. Set $P':=P\cap H$ and consider a facet $\F'$ of $P'$. Then there exists a unique face $\F$ of $P$ of dimension al least $k-1$ such that
\begin{itemize}
\item $\F'=\F\cap H$;
\item $H$  meets $\F$ in its relative interior.
\end{itemize}
\end{lemma}

\proof
The polytope $P$ is defined by a collection of inequalities $\{x \in W \ |\ a_i x \le b_i,\ i=1, \ldots t \}$, with $a_i,b_i \in \qq^d$, $t \ge n+1$ and $H$ is defined by $\{x \in W \ | \ c_j x = d_j, \ j=1,\ldots, d-k\}$, with $c_j,d_j \in \qq^d$. The facet $\F'$ is then defined, up to reordering the coefficients $a_i$'s and $b_i$'s, by $\{x \in W \ |\ a_i x = b_i,\ i=1, \ldots l, \  a_i x \le b_i,\ i=l+1, \ldots t,  \ c_j x = d_j, \ j=1,\ldots, d-k\}$, with $l\le n-k+1$. The set $\{x \in W \ |\ a_i x = b_i,\ i=1, \ldots l, \  a_i x \le b_i,\ i=l+1, \ldots t\}$ defines the unique face $\F$ of $P$ of dimension at least $k-1$ with the required properties.
\endproof

If we now consider the action of a subgroup of automorphisms of the polytope on the vertices $V(P)$, we obtain the following lemma.


\begin{lemma}\label{lemma_convex_2}
Let $P$ be an $n$-dimensional polytope in an affine space $W\simeq\qq^n$ and let $G$ be a finite subgroup of $\GL(W,\qq)$. Assume that $P$ is invariant for the action of $G$ on $W$ and that $W^G$ is $k$-dimensional and intersects the interior of $P$. Then the action of $G$ on the vertices $V(P)$ has at least $k+1$ orbits.
\end{lemma}

\proof
We prove this lemma by induction on $k$.
In the case $k=1$, the fixed locus $W^G$ is a line, which meets two distinct (possibly not maximal) faces $\F_1$ and $\F_2$ of $P$. We immediately obtain two invariant sets: 
$$V(\F_1)\setminus V(\F_2),\mbox{ \ \ and\ \ }V(\F_2)\setminus V(\F_1).$$ 
These give at least two orbits.
\\We prove now the inductive step. Since the intersection of a convex polytope with an affine space is again a convex polytope, we can consider the intersection polytope $P':=P\cap W^G$. Let $\F'$ be one of its ($k-1$-dimensional) facets. Using Lemma \ref{lemma_convex_1}, we can find a (unique) face $\F$ of $P$, cut in its interior by $W^G$ in a $k-1$ affine space. Let $H$ be the smallest affine subspace containing $\F$; it is preserved by the action of $G$. By induction, we obtain at least $k$ orbits. The extra orbit is obtained by the vertices of $P$ not contained in $\F$.
\endproof


\proof[Proof of Theorem \ref{cor_kstability}]
Any smooth Fano toric variety is rigid (cf. \cite[Corollary 4.6]{dFH12}), so we can apply Theorem \ref{rigidchar}: $F$ is fibre-like if and only if $\dim N^1(F)_{\qq}^{\Aut(F)}=1$. 

After tensoring by $\qq$ the exact sequence (\ref{toricses2}), we obtain
 \begin{equation}\label{toricses_q}
 0\rightarrow M_\qq \rightarrow \mathbb{Q}^{V(\De)} \rightarrow N^1(F(\Delta))_\qq \rightarrow 0,
 \end{equation}
where $M_\qq$ is the $n$-dimensional $\mathbb{Q}$-vector space containing the dual polytope of $\Delta$. There is a natural action of $\Aut(\Delta)$ on $M_\qq$ and $\qq^{V(\Delta)}$, and a natural homomorphism $\Aut(\Delta) \to \Aut(F)$, which make the sequence above equivariant for $\Aut(\Delta)$. Moreover by \cite[Corollary 4.7]{Cox95}) we have $N^1(F)_\qq^{\Aut(\Delta)}=N^1(F)_\qq^{\Aut(\F)}$. We need the following general observation.

\begin{lemma}\label{lemma_rep}
Let $G$ be a finite group and $S$ a finite $G$-set. Call $t$ the number of orbits of the action of $G$ on $S$. Let
\[0\rightarrow A \rightarrow \mathbb{Q}^{S} \rightarrow B \rightarrow 0\]
 be an equivariant exact sequence of $\qq$-vector spaces with a $G$-action.
Then 
$$  \dim B^G=t-\dim A^G. $$
\end{lemma}
%LEVEREI I PROSSIMI DUE PARAGRAFI SOSTITUENDOLI CON QUELLI SCRITTI SOTTO
%Let now $G$ be $\Aut(\De)$ and $t$ be the number of orbit of the action of $G$ on $V(\De)$. Lemma \ref{lemma_rep} implies that $F$ cannot be fibre-like if the action of $G=\Aut (\De)$ on $V(\Delta)$ has strictly more than $k+1$ orbits ($k$ here is the dimension of $M^G$). So, using Theorem \ref{berg} the theorem reduces to prove that if $V(\De)$ has exactly $k+1$ orbits, then the barycentre of $\De$ is the origin. 

%Since $F$ is fibre-like, we know that $\dim M^G =k$. We are working over the complex numbers, so the dual representation $N^G$ of the finite group $G$ has the same dimension as $M^G.$ Consider $N^G$ as a $k$-linear subspace cutting the polytope $\De$. 

%RISCRIVEREI DAL LEMMA A QUI IN QUESTO MODO

Let now $G$ be $\Aut(\De)$ and $t$ be the number of orbits of the action of $G$ on $V(\De)$. Set $k:=\dim M^G$; Lemma \ref{lemma_rep} and the exact sequence (\ref{toricses_q}) imply that $F$ is fibre-like if and only if $t-k=1$. If $k=0$ we are done, since the transitive action on the vertices implies the thesis. Therefore, we can assume $k>0$ and want to prove that  if $G$ has exactly $k+1$ orbits on $V(\De)$, then the barycentre of $\De$ is the origin.


%
%FINE DELLA PROPOSTA DI CAMBIO; FORSE ORA METTEREI UN LEMMA DEL TIPO
%
%\begin{lemma}
%Let $k:=\dim M^G$ and assume that $G$ has exactly $k+1$ orbits on $V(\De)$; then any set of $k$ orbits in $V(\De)$ is contained in a face. More explicitly, given $k$ $G$-orbits in $V(\De)$, there exists a face $\F$ of $\De$ such that all these orbits are contained in $V(\F)$.
%\end{lemma}
%\begin{proof}

Since we are working with $\mathbb{Q}$-vector spaces, $M$ and $N$ are isomorphic as $G$-modules; in particular $\dim N^G=\dim M^G=k$.

Let $\De'$ be the intersection polytope $N^G\cap \De$. For every facet $\F'$ of $\Delta'$, one can apply Lemma \ref{lemma_convex_1} to find a unique face $\F$ of $\De$ cut by $N^G$ in its interior. Lemma \ref{lemma_convex_2} says that $V(\F)$ splits in at least $k$ orbits.
Since $F$ is fibre-like, $V(\F)$ splits in exactly $k$ orbits: another orbit is given by the set of vertices $V(\De)\backslash V(F)$.

Let now $\F'_1$ and $\F'_2$ be two distinct facets of $\De'$, which correspond to two faces $\F_1$ and $\F_2$ of $\De$ and determine two sets of $k$ orbits $S_1$ and $S_2$ in $V(\De)$. We claim that $S_1 \neq S_2$: otherwise 
$$V(\F_1) = \bigcup S_1 = \bigcup S_2 = V(\F_2),$$ 
which would imply $\F_1 = \F_2$.

Since there are exactly $k+1$ ways to choose $k$ elements in a set of cardinality $k+1$ and $\De'$ has at least $k+1$ facets (actually exactly $k+1$ by the above argument), we conclude that any collection of $k$ orbits is supported on a face $\F$ of $\De$.


%SO FAR, FOR EACH FACET $\F'$ OF $\De'$ WE HAVE PRODUCED A COLLECTION OF $K$ ORBITS SUPPORTED ON A FACE $\F$ OF $\De$; MOREOVER, GIVEN TWO DIFFEREN FACETS OF $\De'$, WE HAVE SHOWN THAT THE TWO COLLECTIONS ARE DIFFERENT. RECALL THAT THERE ARE EXACTLY $k+1$ ORBITS FOR THE ACTION OF $G$ ON $V(\De)$ AND $\De'$ HAS AT LEAST $K+1$ FACETS; SINCE THERE ARE JUST $K+1$ WAYS TO CHOOSE $K$ ELEMENTS IN A SET OF CARDINALITY $K+1$, WE OBTAIN THE CLAIM.

%\end{proof}


 
Let $\mathcal{P}$ be a primitive collection with trivial focus, whose existence is guaranteed by Proposition \ref{batyrev}. Since any set of $k$ orbits must be contained in a face, $\mathcal{P}$ must involve at least one vertex from every orbit. Acting with $G$ on $\mathcal{P}$ we obtain a  family of primitive collections $\{ \mathcal{P}_i \}_{1\le i \le r }$ such that $\sigma(\mathcal{P}_i)=0$ and $\cup \mathcal{P}_i=V(\De)$. Assume that $\mathcal{P}_i \cap \mathcal{P}_j \ne \emptyset$ for some $i,j$, i.e. $\mathcal{P}_i=\{x_1, \ldots, x_k\}$ and $\mathcal{P}_j=\{x_1, \ldots, x_h, y_{h+1}, \ldots ,y_k\}$ with $y_s \ne x_t$ for any $s,t$. Then 
$$
x_{h+1}+\ldots +{x_k}=y_{h+1}+\ldots y_k,
$$ 
which is impossible by Remark \ref{rmk}, because $x_{h+1}, \ldots, x_k$ generate a cone in $\Sigma$.


This implies that all the $\mathcal{P}_i$'s are disjoint and, as a consequence, that the sum of all vertices of $\De$ equals the origin, i.e. the barycentre of $\De$ is trivial. The theorem is proved.
\endproof

%Let us remark that there are many smooth toric Fanos which are $K$-stable but not fibre-like.
The previous corollary seems to be the relative version in the toric case of the following very general conjecture by Odaka and Okada.

\begin{con}[{\cite[Conj. 5.1]{OO13}}]
Any smooth Fano manifold $X$ of Picard rank 1 is  $K$-semistable.
\end{con}

\subsection{MAGMA computations}

Theorem \ref{cor_kstability} and its proof show that the fibre-like condition is rather restrictive.
\\The following table collects the smooth Fano toric varieties (up to dimension 8) which are fibre-like. It has been obtained using the software MAGMA together with the Graded Ring Database \cite{GRDB} (for further details on the classification, cf. \cite{Obro}).
In the following table, the IDs of the Fano polytopes are the ones introduced in \cite{GRDB}.

 %We note that the only varieties we are not able to classify are the ID 5817, 277415 and 830429. 

{
\begin{displaymath} \label{t1} 
\begin{array}{cccc} 
 \mbox{Dimension} & \#\mbox{Vertices} & \mbox{Description}  & \mbox{ID}  \\
\hline 
\hline
 2  & 6 & V_2  & 2  \\
 2 &  4 & \pp^1 \times \pp^1  & 4  \\
  2 &  3 & \pp^2  & 5 \\
\hline
 3 & 6 & (\pp^1)^3  & 21   \\
 3 & 4 & \pp^3 &  23     \\
\hline
4 &  10 & V_4  & 63   \\
4 & 12 & V_2 \times V_2  & 100 \\
4 & 8 & (\pp^1)^4  & 142  \\
4 & 6 & \pp^2 \times \pp^2  & 146    \\
4 & 5 & \pp^4  & 147    \\
\hline
5 & 10 & (\pp^1)^5  & 1003    \\
5 & 6 & \pp^5  & 1013    \\
\hline
6 &  14 & V_6  & 1930   \\
6 & 12 & W_1  & 5817 \\
6 & 18 & (V_2)^3  & 7568  \\
6 & 12 & (\pp^1)^6  & 8611  \\
6 & 9 & (\pp^2)^3  & 8631    \\
6 & 8 & (\pp^3)^2  & 8634    \\
6 & 7 & \pp^6  & 8635    \\
\hline
7 & 14 & (\pp^1)^7  & 80835    \\
7 & 8 & \pp^7  & 80891   \\
\hline
8 & 18 & V_8  & 106303   \\
8 & 15 & W_2  & 277415  \\
8 & 20 & (V_4)^2  & 442179  \\
8 & 24 & (V_2)^4  & 790981  \\
8 & 12 & W_3  & 830429    \\
8 & 16 & (\pp^1)^8	  & 830635    \\
8 & 12 & (\pp^2)^4  & 830767    \\
8 & 10 & (\pp^4)^2  & 830782    \\
8 & 9 & \pp^8  & 830783    \\
 \end{array} 
\end{displaymath}
%\captionof{table}{}
}



\begin{rem}\label{super_skansen}
The varieties $V_d$ are known as Del Pezzo varieties (see \cite{VK85} for more details). There is no classical description for the varieties $W_1,W_2$ and $W_3$. %We just note  the action of the automorphism group $\Aut(\De)$ is transitive on the vertices.
\end{rem}


We would like to finish off by stating the following speculation.

\begin{con}
Let $\De$ be a smooth fibre-like polytope of dimension $d$. Assume that $d$ is an odd prime number.  Then either $X(\De)=\pp^d$ or $X(\De)=(\pp^1)^d$.   
\end{con}







